Notes on the Theory of Statistical Symbol Recognition

This document is a pdf generated from old plain-TeX files of 1986, of Nils Lid Hjort's `Notes on the Theory of Statistical Symbol Recogntion', a limited circulation 207-pages monograph published at the Norwegian Computing Centre, as Report no. 778/1986. It gives the basics of the statistical pattern recognition theory developed to suit the needs of several industrial projects, related to contracts with the Norwegian-German firm SysScan, the Royal Norwegian Research Council, and yet others, involving symbol recognition and classification analysis from noisy images, related to maps, documents, satellite imaging, etc. The methods and algorithms developed also needed to fit the technology of that time, anno c. 1986, with machines scanning documents, converting these to vector representation, within computational and machine system boundaries. There is an accompanying and also limited circulation booklet, `Statistical Symbol Recognition: Development of a System', by Knut Br{\aa}ten, Erik Holb{\ae}k-Hanssen, and Torfinn Taxt (Report No.777/1986, Norwegian Computing Centre, Oslo), detailing the system developments. Thus developments took form and shape on two frontiers, in close collaboration, Hjort's statistical methods and getting the technology to work, with its multiple components, hardware and software.

==> texini.tex <==
%------------------------------------------------------------------------------
%
% Definisjoner til TeX, laget av Jacson                        Versjon 1-jul-86
%
%------------------------------------------------------------------------------
%
% Generelt.
%
% Denne filen er lagt p} ted: slik at (nye) brukere av TeX kan kopiere den til
% eget omr}de og forandre/forbedre/bruke den etter eget |nske. Vi tar ikke
% ansvar for at definisjonene er feilfrie. De er helt sikkert ikke spesielt
% smarte, og viser nok ikke beste m}te } gj|re ting p} i alle samenhenger.
%
% For videre informasjon, se:
%
%    TeXbook             (Spiralutgave i Bokhandelen)
%    ABC om TeX          (Gratis hefte fra USE, Ekspedisjonen)
%    doc:texuio.tex      (Kilden til neste fil:)
%    doc:texuio.dvi      (Kan tas ut direkte med WRITE p} Laser)
%    NUSE-artikler 
%
% Videre foreligger f|lgende b|ker:
%
%    LaTeX Users Guide   (LaTeX er en makropakke laget med TeX)
%    The Joy of TeX      (Manual for AMSTeX, an makropakke laget med TeX)
%    The Metafont book   (Manual for Metafont, spiralinnbinding)
%
% Et fembinds innbundet verk om TeX og Metafont er utgitt av Addison Wesley.
% Her inng}r The TeX book og The Metafont book, samt to bind med programkode
% samt et bind med definisjonene og programmene for alle tegnene i Computer
% Modern fontene. Et must for TeXnikkere!
%
%------------------------------------------------------------------------------
%
% Bruk
%
% Hvis man bruker denne filen, eller lager en tilsvarende selv, vil starten p}
% .tex-filen naturlig se slik ut:
%
%    \input norsk
%    /input texini       (eventuelt ted:texini)
%    /hsize...
%    /vsize...
%    /output-rutine     (hvis ikke /plainoutput skal brukes)
%    -lokale /def-
%    -Tekst-
%
%------------------------------------------------------------------------------
%
% Innhold
%
%    A. Fonter
%    B. Innramming av bokser
%    C. Kapitler, seksjoner osv m/automatisk nummerering
%    D. Tegning av taster
%    E. Automatisk generering av innholdsfortegnelse
%    F. Items
%    G. Tomme-angivelse
%    H. Ordreoppsett i /tt
%    I. Stor f|rstebokstav i nytt kqpittel
%    J. Noen logoer
%    K. /hfuzz
%    L. Sitater
%    M. Nytt kapittel som odde side
%    N. Diverse skip og lim
%    O. Fotnoter
%    P. Overf|ring av sidenummer mellom filer
%    Q. Horisontale streker i /halign-tabeller
%    R. QED
%    S. Noen definisjoner fra NUSE
%    T. Hakeparenteser
%    U. Noen parametre
%    V. Eksempel p} /output-rutine
%
%------------------------------------------------------------------------------
%
% A) Fonter.
%
% Dette er fonter jeg bruker i mitt arbeid, bytt ut mine font-definisjoner med
% egne etter behov.
%
% NB! V{r varsom ved bruk av /mag; de aller fleste fontene her skulle g} bra 
% ved /mag/magstep1. Ved /mag/magstehalf fins ikke /slen, /slto, /csc.
%
%/font/fontmeta = manfnt                 % Spesiell font
/font/sixrm    = cmr6                   % 6 pt Roman
/font/ninerm   = cmr9                   % 9 pt Roman   (f.eks. fotnoter)
/font/ninesl   = cmsl9                  % 9 pt Slanted (f.eks. fotnoter)
/font/rmen     = cmr10 scaled/magstep1  % Forst|rrelse av 10 pt Roman
/font/rmto     = cmr10 scaled/magstep2  %  --
/font/rmtre    = cmr10 scaled/magstep3  %  --
/font/rmfire   = cmr10 scaled/magstep4  %  --
/font/rmfem    = cmr10 scaled/magstep5  %  --
/font/rmseks   = cmr10 scaled 2986      %  --
%/font/rmbig    = cmsmc4                 % Meget store bokstaver (40 pt)
/font/bfen     = cmbx10 scaled/magstep1 % Forst|rrelse av 10 pt Boldface
/font/slen     = cmsl10 scaled/magstep1 % Forst|rrelse av 10 pt Slanted
/font/iten     = cmitt10 scaled/magstep1% Forst|rrelse av 10 pt Italics
/font/csc      = cmcsc10                % Caps Small Caps (kun versatiler)
%
%------------------------------------------------------------------------------
%
% B) Innramming av bokser.
%
% Hvis man har en boks /minboks, rammes den inn med f.eks.:
%
%    /thinbox</box/minboks>
%
/def/thinbox#1</vbox</hrule/hbox</vrule/hskip 4pt/vbox
    </vskip 4pt #1 /vskip 4pt>/hskip 4pt/vrule>/hrule>>
/def/medbox#1</vbox</hrule height 1pt/hbox</vrule width 1pt/hskip 6pt
    /vbox</vskip 6pt #1/vskip 6pt>/hskip 6pt/vrule width 1pt>/hrule height 
    1pt>>
/def/fatbox#1</vbox</hrule height 3pt/hbox</vrule width 3pt/hskip 10pt
    /vbox</vskip 10pt #1/vskip 10pt>/hskip 10pt/vrule width 3pt>/hrule height 
    3pt>>
%
%------------------------------------------------------------------------------
%
% C) Kapitler og avsnitt med automatisk nummerering.
%
%    1         /chapter
%    1.1       /section
%    1.1.1     /subsection
%    1.1.1.1   /subsubsection
%
% Skriv f.eks.:
%   
%    /section Innledning
%
% med blank linje etter (/par avslutter  parameteren i definisjonene)
%
% F|rst kommer endel hjelpdefinisjoner
%
/let/A=/let /let/B=/let /let/C=/let /let/X=/let
/def/noeject</vadjust</nobreak>>
/def/headnobreak#1</allowbreak/noindent<#1>/noeject
    /smallskip/nobreak/noindent/ignorespaces>
/count1=0
/count4=0
/def/nc#1</number/count#1>
/def/rc#1</romannumeral/count#1>
/def/prt#1</par/advance/count4 by 1/centerline</rmto #1>/biggskin>
/def/chap#1</par/advance/count1 by 1/count2=0
    /biggskip/headnobreak</bfen/nc1/ / #1>>
/def/sect#1</par/advance/count2 by 1/count3=0
    /bigskip/headnobreak</bf/nc1./nc2/ / #1>>
/def/part#1/par</prt<#1>/content<</rmto #1>><</rmen /nc1>></X>%
    /ignorespaces/biggskin>
%
% Hoveddefinisjonene
%
/def/chapter#1/par</chap<#1>/content<</bf #1>><</bf /nc1>></A>%
    /ignorespaces>
/def/section#1/par</sect<#1>/content<#1></nc1./nc2></B>%
    /ignorespaces>
/def/subsection#1/par</advance/count3 by 1/count4=0
    /medskip/headnobreak</bf/nc1./nc2./nc3/ / #1>%
    /content<#1></nc1./nc2./nc3></C>/ignorespaces>
/def/subsubsection#1/par</advance/count 4 by 1/count5=0
    /medskip/headnobreak</bf/nc1./nc2./nc3./nc4/ / #1>/ignorespaces>
%
%------------------------------------------------------------------------------
%
% D) Tegning av taster 
%
% Skriv f.eks.:
%
%    /tast<CR>
%
/def/tastbox#1</vbox</hrule/hbox</vrule/hskip 1pt/vbox
    </vskip 1pt #1 /vskip 1pt>/hskip 1pt/vrule>/hrule>>
/def/tast#1</leavevmode/hbox</tastbox</hbox</sixrm #1>>>>
%
%------------------------------------------------------------------------------
%
% E) Generering av innholdsfortegnelse:
%
% Innholdsfortegnelsen genereres p} en egen fil som kan kj|res gjennom TeX
% etterp}, f.eks. ved } bruke kommandoen
%    
%    /con
%
% helt tilslutt (foran /end). Da kommer innholdsfortegnelsen ut som siste side.
% F|lgende definisjoner inng}r:
%
%    /content             Plasserer et entry i innholdsfortegnelsen
%    /A/B/C...            Design for linjene som skrives ut
%    /con                 Henter innholdsfortegnelsen fra filen
%    /topofcontents       Start p} f|rste side av innholdsfortegnelsen
%    /botofcontents       Slutten p} sidene med innholdsfortegnelse
%    /contentspagenumber  Sidenummer til innholdsfortegnelsen
%    /contentsfile        Navn p} filen med innholdsfortegnelse
%    /newwrite            Definerer filen
%    /openout             ]pner filen for skriving
%
/def/content#1#2#3<</let]=/let /let}=/let /let/TeX=/let /let/slash=/let
    /let/AmSTeX=/let /let/"=/let /let/`=/let
    /edef/writeit</write/cont<#3<#1>%
    </noexpand/number/count0><#2>>>/writeit>>
/def/topofcontents</vfill/centerline<</bf INNHOLD>>/bigskip
    /line</hfil Side>/medskip>
/def/botofcontents</vfill> 
/def/contentspagenumber<0> 
/def/contentsfile<CONTENTS>             % NB! Ikke /eject rett f|r /con
/def/con<
    /write/cont<>                       % S|rg for at filen ikke er tom
    /closeout/cont                      % All informasjon er samlet inn
    /par/vfill/eject                    % Start side for innholdsfortegnelse
    /rightskip 0pt/hyphenpenalty 50/tolerance 200
    /output</shipout/vbox</box255>>
    /count0=/contentspagenumber
    /topofcontents
/def/A##1##2##3</medskin
    /line</hbox to 30pt<##3/hfil>/ignorespaces</bf ##1>% 
    /leaders/hbox to .5em<./hfil>/hfil/ ##2>>
/def/B##1##2##3<
    /line</hbox to 30pt<##3/hfil>/ignorespaces ##1% 
    /leaders/hbox to .5em<./hfil>/hfil/ ##2>>
/def/C##1##2##3<
    /line</hskip 30pt/hbox to 30pt<##3/hfil>/ignorespaces ##1% 
    /leaders/hbox to .5em<./hfil>/hfil/ ##2>>
/def/X##1##2##3</biggskin/line</hfil ##1/hfil>/medskin>
/message<Table of contents:>
/input/contentsfile/relax               % Les inn innholdsfortegnelsen
/botofcontents>            
/newwrite/cont                          % Skriv ut innholdsfortegnelsen
/immediate/openout/cont=/contentsfile
%
%------------------------------------------------------------------------------
%
% F) Items
%
% Skriv f.eks.:
%
%    /ik Tekst
%
% og f} items med kuler foran.
%
/def/kule<$/bullet$>
/def/ik</item</kule>>
/def/iik</itemitem</kule>>
/def/iis</itemitem<-->>
%
%------------------------------------------------------------------------------
%
% G) Tomme-angivelse (nyttig n}r man f.eks. skal skrive om disketter e.l.
%
/def/tommer#1<$#1^</prime/prime>$>
%
%------------------------------------------------------------------------------
%
% H) Ordreoppsett
%
% NB! Bredden p} /ordrebox m} eventuelt endres etter behov.
%
% Skriv f.eks.:
%
%    /orders<F|rste ordrelinje/lf
%    Andre ordrelinje>
%
% (NB! Kan forbedres!!)
%
/def/lf</hfil/break>
/newbox/ordrebox
/def/orders#1</medskin/setbox/ordrebox/vbox</hsize10.5truecm
    /obeylines/tt/parskip0pt/noindent #1>%
    /hskip/the/parindent/box/ordrebox/medskin/ignorespaces>
%
%------------------------------------------------------------------------------
%
% I) Stor bokstav f|rst i avsnitt, f.eks. i begynnelsen av et nytt kapittel
%
% Skriv f.eks.:
%
%    /fancy Tekst....
%
% som start p} et avsnitt.
%
/newbox/fanebox
/def/fancy#1</setbox/fanebox/hbox<%
    /lower 12pt/hbox</rmseks #1>/hskip 6pt>/dp/fanebox=0pt
    /begingroup/clubpenalty=10000/def/par</endgraf/endgroup>%
    /hangindent /wd/fanebox/hangafter=-2
    /noindent/hskip -/wd/fanebox/box/fanebox
    /hskip -6pt>
%
%------------------------------------------------------------------------------
%
% J) Noen logoer.
%
%    /LaTeX
%    /AMSTeX
%    /MF        METAFONT
%    /AbC       For USE's ABC-hefter, ABC med nedsenket B
%    /SPSSX     
%
/def/AMSTeX<$/cal A/kern-.1667em/lower.5ex/hbox<$/cal M$>/kern-.125em S$-/TeX>
/def/MF<</fontmeta hijklmnj>>
/def/LaTeX<L/kern-2.5pt/raise2.5pt/hbox</ninerm a>/TeX>
/def/AbC<A/kern -.12em/lower .3ex/hbox<B>/kern -.1em C>
/def/SPSSX<SPSS/raise0.8ex/hbox<x>>
%
%------------------------------------------------------------------------------
%
% K) Undertrykk meldinger om bokser som er mindre enn 2.5pt overfulle
%
/hfuzz 2.5pt
%
%------------------------------------------------------------------------------
%
% L) Sitater
% 
% Disse skrives ut indentert i begge marger, i 9pt stil, og med anf|rselstegn
% foran og bak.
%
%    /citat       Korte sitater, kun en paragraf
%    /citatlong   Lengre sitater, flere paragrafer, kan brytes mellom sider
%    /citd        Hakeparenteser med tre prikker inni
%
% Skriv f.eks.:
%
%    /citat<Tekst>
%
/def/cit#1</char"5B #1/char"5D/ >
/def/citd</cit<$/ldots$>>
/def/citat#1</medskip/vbox</baselineskip11pt/narrower/ninerm/noindent
    /llap<``/thinspace>#1''/par>/medskip>
/def/citatlong#1</medskip</narrower/baselineskip11pt/ninerm/noindent
    /llap<``/thinspace>#1''/par>/medskip>
%
%------------------------------------------------------------------------------
%
% M) Ekstra side slik at nye kapitler starter som odde side (h|yre-side).
%
% Legges inn i /output-rutinen som en test
%
/def/extrapage</ifodd/pageno/else/vbox to 5cm<>/vfill/eject/fi>
%
%------------------------------------------------------------------------------
%
% N) Diverse skip og lim
%
%    /smallskin     Tilsvarer /smallskip/noindent
%                   (Ditto /medskin osv.)
%    /smallneg      Tilsvarer negativ /smallskip
%                   (Ditto /medneg osv.)
%    /biggskip      Det dobbelte av /bigskip
%                   (Ditto /biggskin, /biggneg)
%
% Eksempel p} bruk av negativt lim: Hvis man f.eks. skriver:
%
%    /chapter Overskrift
%
%    /section Overskrift
%
% alts} hvis avsnittet starter rett etter kapitteloverskriften, blir avstanden
% mellom de to overskriftene for stor, og man kan legge inn passende negativt
% lim imellom:
%
%    /chapter Overskrift
%
%    /bigneg
%
%    /section Overskrift
%
/newskip/biggskipamount
/biggskipamount=24pt plus4pt minus4pt
/def/biggskip</bigskip/bigskip>
/def/smallskin</smallskip/noindent>
/def/medskin</medskip/noindent>
/def/bigskin</bigskip/noindent>
/def/biggskin</biggskip/noindent>
/def/smallneg</vskip-/smallskipamount>
/def/medneg</vskip-/medskipamount>
/def/bigneg</vskip-/medskipamount>
/def/biggneg</vskip-/biggskipamount>
%
%------------------------------------------------------------------------------
%
% O) Fotnoter
%
%    /fotnote    Nederst p} siden, med automatisk nummerering
%    /baknote    Notene skal bakerst, i teksten markeres de kun, og de m}
%                skrives inn bakerst, f.eks. med /item e.l.
%
% Skriv f.eks.:
%
%    Tekst/fotnote<Fotnotetekst>Mer tekst
%   
%    Tekst/baknote<14>Mer tekst
%
/newcount/footnotecount
/footnotecount=1
/def/fotnote#1</footnote<$^</number/footnotecount>$>%
    </ninerm/baselineskip11pt#1>/global/advance/footnotecount by 1>
/def/baknote#1<$^<#1>$>
%
%------------------------------------------------------------------------------
%
% P) Overf|ring av sidenummer mellom filer.
%
% Nyttig ved store manus hvor man vil ha f.eks. kapitlene som separate filer.
% Brukes ved at en fil avsluttes med:
%
%    /skrivpageno/end
%
% og neste fil starter med:
%
%   /lespageno<forrige>
%
% der forrige er navnet p} forrige fil. Sidenumrene overf|res v.hj.a. filer
% med extension .pno. N}r manus er splittet p} flere filer, kan ikke /con
% brukes for } generere innholdsfortegnelse, men pno-filene inneholder side-
% tallene for kapittelstart, slik at man manuelt kan sette sammen en innholds-
% fortegnelse.
%
/newwrite/Page
/def/skrivpageno</extrapage/vfill/supereject
    /immediate/openout/Page=/jobname.pno 
    /immediate/write/Page</number/pageno>
    /immediate/closeout/Page>
/def/lespageno#1</pageno=/input #1.pno>
%
%------------------------------------------------------------------------------
%
% Q) Horisontale streker i tabeller som er indentert
%
% Ofte vil /hrule brukt inni /halign (med /noalign</hrule>) stikke ut i venstre
% marg dersom /halign gj|r en /indent.
%
%    /noa    Strek indentert /parindent
%    /noal   Strek indentert som angitt parameter
%
/newdimen/lengde
/lengde=/the/hsize
/advance/lengde -/the/parindent
/def/noa</noalign</smallskip/nointerlineskip/moveright/the/parindent
    /vbox</hrule width/lengde>/nointerlineskip/smallskip>>
/def/noal#1</noalign</smallskip/nointerlineskip/moveright/the/parindent
    /vbox</hrule width#1>/nointerlineskip/smallskip>>
%
%------------------------------------------------------------------------------
%
% R) Svart boks f.eks. til avslutning av bevis, eksempler e.l.
%
/def/QED</hskip2pt/vrule height4pt width3pt depth2pt>
%
%------------------------------------------------------------------------------
%
% S) Fra NUSE.
%
%    1. Innrammet artikkel (h|yst en side), brukes slik:
%
%    /beginframe   
%
%    Tekst
%
%    /endframe
%
/newbox/notabene
/newbox/lederbox
/def/endframe</medskip>
/long/def/beginframe#1/endframe</setbox/notabene/vbox</narrower #1/par>%
     /centerline</medbox</box/notabene>>>
%
%    2. Artikkel-heading, brukes slik:
%
%    /beginheading Navn
%
%    /title s; Tekst;
%    /title s; Tekst;
%
%    /endheading
%
%    der:  s=1   /rmen
%          s=2   /rmto
%          s=3   /rmtre
%          s=4   /rmfire
%          Navn  Forfatternavn
%          Tekst Artikkelens overskrift
%
%    Vilk}rlig antall tittel-linjer. Ikke glem semikolonene!
%
/newskip/tskipamount
/def/tskip</vskip/tskipamount>
/def/leaderfill</quad/leaders/hrule height1pt/hfill>
/def/beginheading#1/par</line<</slto #1>/leaderfill>/medskip>
/def/title#1;#2;</ifcase#1/or /let/rmcurrent=/rmen
                              /tskipamount=/smallskipamount
                          /or /let/rmcurrent=/rmto
                              /tskipamount=/smallskipamount
                          /or /let/rmcurrent=/rmtre
                              /tskipamount=/medskipamount
                          /or /let/rmcurrent=/rmfire
                              /tskipamount=/bigskipamount
                          /or /let/rmcurrent=/storfont
                              /tskipamount=/bigskipamount
                          /else /let/rmcurrent=/csc
                                /tskipamount=/medskipamount/fi
    /centerline</rmcurrent #2>/tskip>
/def/endheading</medskip/hrule height1pt/biggskin>
%------------------------------------------------------------------------------
%
% T) Hakeparenteser
%
/def/lb<$/lbrack$>
/def/rb<$/rbrack$>
%
%------------------------------------------------------------------------------
%
% U) To parametre som henger sammen med /output-rutinene og som eventuelt m}
%    sl}s av eller p} etter behov.
%
%    /titletrue   Ikke sidehode p} f|rstesider i nytt kapittel
%    /ekstrapage  Nytt kapittel p} odde sider
%
%/titletrue
/extrapage
%
%------------------------------------------------------------------------------
%
% V) Output-rutine
%
% Nedenfor gjengis et eksempel p} en selvlaget /output-rutine som jeg bruker
% til USE's ABC-hefter. Rutinen ligner mye p} /plainoutput. Mine endringer er
% hovedsaklig f|lgende.
%
%    - Selvlaget sidehode som veksler med venstre- og h|yresider 
%    - Endret sidebunn (tatt bort sidenummer)
%    - Tester p} /titletrue og /ekstrapage
%
% F|lgende st|rrelser inng}r:
%
%    /dokutitle    Tekst som skal |verst p} hver side
%    /output       Tar med noen ekle tegn, og kaller inn /plainoutput
%    /titlebox     Boks for teksten |vert p} sidene
%    /sidenr       Sidenummer
%    /heading      Boks for hele sidehodet
%    /dropbody     Avstand mellom sidehodet og sidens innhold
%    /iftitle      Test p} om dette er en f|rsteside
%    /nonumb       test p} om det skal v{re sidetall nederst p} sidene
%
% Merk at /plainoutput i hovedsak er definert som (se TeXbook s. 225-226)
%
%    /makeheadline
%    /pagebody
%    /makefootline
%    /advancepageno
%    /eject
%
% og at definisjonene nedenfor endrer p} /makeheadline og /makefootline.
% mesteparten av koden g}r med til } endre /makeheadline, idet det skal
% skilles mellom venstre- og h|yresider, og noen bokser skal limes sammen.
%
% Eksempel p} resultat finnes f.eks. i ABC om USE's Tilbud og Tjenester 1986.
%
% /def/dokutitle</AbC/ om USE's tilbud og tjenester>
% /output=</let]=/let /let/TeX=/let /let/"=/let /let/`=/let /plainoutput>
% /newbox/titlebox
% /newbox/sidenr
% /newbox/heading
% /newdimen/dropbody
% /newif/iftitle
% /newif/ifnonumb
% /setbox/titlebox/hbox</bf/dokutitle>
% /dropbody=55pt
% /def/makeheadline</sl/iftitle/global/titlefalse/else
%     /setbox/sidenr/vbox to /dropbody</hbox</rmto/number/pageno>/vfill>
%     /dimen0=/hsize/advance/dimen0 by -/wd/sidenr
%     /ifodd/pageno/setbox/heading/vbox to /dropbody</hsize/dimen0
%           /line</copy/titlebox/hfill>
%           /line</firstmark/hfill>/vfill>
%           /line</box/heading/hss/box/sidenr>
%     /else /setbox/heading/vbox to /dropbody</hsize/dimen0
%           /line</hfill/copy/titlebox>
%           /line</hfill/firstmark>/vfill>
%           /line</box/sidenr/hss/box/heading>
%     /fi/fi
%     >
% /def/makefootline</ifnonumb/global/nonumbfalse/line<>/else
%     /baselineskip24pt/line</the/footline>/fi>
%
%------------------------------------------------------------------------------
%
% - Slutt -
%
%------------------------------------------------------------------------------

